Seven challenges for harmonizing explainability requirements

Regulators have signalled an interest in adopting explainable AI(XAI) techniques to handle the diverse needs for model governance, operational servicing, and compliance in the financial services industry. In this short overview, we review the recent technical literature in XAI and argue that based on our current understanding of the field, the use of XAI techniques in practice necessitate a highly contextualized approach considering the specific needs of stakeholders for particular business applications.

==> Makefile <==
MAIN=main
BIB=bib
OUTPUT_DIR=output
AUX_DIR=output_aux

.PHONY: all check link clean travis data tatoeba

pdf:
	latexmk -pdf $(MAIN) -auxdir=$(OUTPUT_DIR) -outdir=$(OUTPUT_DIR)

all: pdf
	make -C code/programs

check:
	chktex -n1 -n2 -n3 -n8 -n11 -n12 -n13 -n14 -n26 -n34 -n33 -n36 -n40 -n44 $(MAIN)
	biber --tool -V $(BIB).bib
	rm -f $(BIB)_bibertool.bib

lint:
	biber --tool $(BIB).bib --output-fieldcase=lower --isbn-normalise
	mv $(BIB)_bibertool.bib $(BIB).bib

arxiv: pdf
	mkdir -p arxiv
	cp *.pdf $(OUTPUT_DIR)/*.bbl *.bib *.tex *.cls *.bst arxiv
	#Download any new versions of packages here
	#e.g.
	#curl -L -o arxiv/algorithm2e.sty https://ctan.sharelatex.com/tex-archive/macros/latex/contrib/algorithm2e/tex/algorithm2e.sty
	#Test build
	cd arxiv && latexmk -pdf $(MAIN) -auxdir=arxivtest -outdir=arxivtest && rm -rf arxivtest
	cd arxiv && zip arxiv.zip *

clean:
	latexmk -c -pdf
	rm -rvf *.bbl *.blg *.aux *.fls *.fdb_latexmk *.log *.out *.toc $(MAIN).pdf $(AUX_DIR) $(OUTPUT_DIR) arxiv

travis:
	#Old latexmk doesn't understand auxdir and outdir options
	latexmk -pdf -pdflatex='pdflatex %S %O -interaction=nonstopmode -halt-on-error' $(MAIN)

######################
# Download data
######################
TATOEBA_CORPUS = data/tatoeba/users_sentences.csv \
	data/tatoeba/user_languages.csv \
data/tatoeba/sentences_in_lists.csv \
data/tatoeba/links.csv \
data/tatoeba/tags.csv \
data/tatoeba/sentences_detailed.csv \
data/tatoeba/user_lists.csv

data: $(TATOEBA_CORPUS)

tatoeba: $(TATOEBA_CORPUS)

data/tatoeba/users_sentences.csv:
	curl --create-dirs -R -L -z $@ -o $@ https://downloads.tatoeba.org/exports/users_sentences.csv

data/tatoeba/%.csv: data/tatoeba/%.tar.bz2
	tar -xjvf $< -C data/tatoeba

data/tatoeba/%.tar.bz2:
	curl --create-dirs -R -L -z $@ -o $@ https://downloads.tatoeba.org/exports/$(notdir $@)



==> latexmkrc <==
# Set time zone
# Reference
# https://www.overleaf.com/learn/latex/Articles/How_to_use_latexmkrc_with_Overleaf:_examples_and_techniques
$ENV{'TZ'}='America/New_York';

# Put all the style files here
# Reference
# https://www.overleaf.com/learn/latex/Questions/I%20have%20a%20lot%20of%20.cls,%20.sty,%20.bst%20files,%20and%20I%20want%20to%20put%20them%20in%20a%20folder%20to%20keep%20my%20project%20uncluttered.%20But%20my%20project%20is%20not%20finding%20them%20to%20compile%20correctly
$ENV{'TEXINPUTS'}='./styles//:' . $ENV{'TEXINPUTS'};


# The rest of the file below is copied from
# https://www.overleaf.com/learn/how-to/How_does_Overleaf_compile_my_project%3F
# as of 2019-08-23.

###############################
# Post processing of pdf file #
###############################

# assume the jobname is 'output' for Overleaf v2
my $ORIG_PDF_AGE = -M "output.pdf"; # get age of existing pdf if present

END {
    my $NEW_PDF_AGE = -M "output.pdf";
    return if !defined($NEW_PDF_AGE); # bail out if no pdf file
    return if defined($ORIG_PDF_AGE) && $NEW_PDF_AGE == $ORIG_PDF_AGE; # bail out if pdf was not updated
    my $QPDF = "/usr/bin/qpdf";
    return if ! -x $QPDF; # check that qpdf exists
    my $status = system($QPDF, "--linearize", "output.pdf", "output.pdf.opt");
    my $exitcode = ($status >> 8);
    print "qpdf exit code=$exitcode\n";
    # qpdf returns 0 for success, 3 for warnings (output pdf still created)
    return if !($exitcode == 0 || $exitcode == 3);
    print "Renaming optimised file to output.pdf\n";
    rename("output.pdf.opt", "output.pdf");
}

##############
# Glossaries #
##############
add_cus_dep( 'glo', 'gls', 0, 'glo2gls' );
add_cus_dep( 'acn', 'acr', 0, 'glo2gls');  # from Overleaf v1
sub glo2gls {
	system("makeglossaries $_[0]");
}

#############
# makeindex #
#############
@ist = glob("*.ist");
if (scalar(@ist) > 0) {
        $makeindex = "makeindex -s $ist[0] %O -o %D %S";
}

################
# nomenclature #
################
add_cus_dep("nlo", "nls", 0, "nlo2nls");
sub nlo2nls {
	system("makeindex $_[0].nlo -s nomencl.ist -o $_[0].nls -t $_[0].nlg");
}

#########
# Knitr #
#########
my $root_file = $ARGV[-1];

add_cus_dep( 'Rtex', 'tex', 0, 'rtex_to_tex');
sub rtex_to_tex {
    do_knitr("$_[0].Rtex");
}

sub do_knitr {
    my $dirname = dirname $_[0];
    my $basename = basename $_[0];
    system("Rscript -e \"library('knitr'); setwd('$dirname'); knit('$basename')\"");
}

my $rtex_file = $root_file =~ s/\.tex$/.Rtex/r;
unless (-e $root_file) {
	if (-e $rtex_file) {
		do_knitr($rtex_file);
	}
}

##########
# feynmf #
##########
push(@file_not_found, '^feynmf: Files .* and (.*) not found:$');
add_cus_dep("mf", "tfm", 0, "mf_to_tfm");
sub mf_to_tfm { system("mf '\\mode:=laserjet; input $_[0]'"); }

push(@file_not_found, '^feynmf: Label file (.*) not found:$');
add_cus_dep("mf", "t1", 0, "mf_to_label1");
sub mf_to_label1 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t1"); }
add_cus_dep("mf", "t2", 0, "mf_to_label2");
sub mf_to_label2 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t2"); }
add_cus_dep("mf", "t3", 0, "mf_to_label3");
sub mf_to_label3 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t3"); }
add_cus_dep("mf", "t4", 0, "mf_to_label4");
sub mf_to_label4 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t4"); }
add_cus_dep("mf", "t5", 0, "mf_to_label5");
sub mf_to_label5 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t5"); }
add_cus_dep("mf", "t6", 0, "mf_to_label6");
sub mf_to_label6 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t6"); }
add_cus_dep("mf", "t7", 0, "mf_to_label7");
sub mf_to_label7 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t7"); }
add_cus_dep("mf", "t8", 0, "mf_to_label8");
sub mf_to_label8 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t8"); }
add_cus_dep("mf", "t9", 0, "mf_to_label9");
sub mf_to_label9 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t9"); }

##########
# feynmp #
##########
push(@file_not_found, '^dvipdf: Could not find figure file (.*); continuing.$');
add_cus_dep("mp", "1", 0, "mp_to_eps");
sub mp_to_eps {
    system("mpost $_[0]");
    return 0;
}

#############
# asymptote #
#############
sub asy {return system("asy --offscreen '$_[0]'");}
add_cus_dep("asy","eps",0,"asy");
add_cus_dep("asy","pdf",0,"asy");
add_cus_dep("asy","tex",0,"asy");

#############
# metapost  #  # from Overleaf v1
#############
add_cus_dep('mp', '1', 0, 'mpost');
sub mpost {
  my $file = $_[0];
  my ($name, $path) = fileparse($file);
  pushd($path);
  my $return = system "mpost $name";
  popd();
  return $return;
}

##########
# chktex #
##########
unlink 'output.chktex' if -f 'output.chktex';
if (defined $ENV{'CHKTEX_OPTIONS'}) {
    use File::Basename;
    use Cwd;

    # identify the main file
    my $target = $ARGV[-1];
    my $file = basename($target);

    if ($file =~ /\.tex$/) {
	# change directory for a limited scope
	my $orig_dir = cwd();
	my $subdir = dirname($target);
	chdir($subdir);
	# run chktex on main file
	$status = system(
    "/usr/bin/run-chktex.sh",
    $orig_dir,
    $file
  );
	# go back to original directory
	chdir($orig_dir);

	# in VALIDATE mode we always exit after running chktex
	# otherwise we exit if EXIT_ON_ERROR is set

	if ($ENV{'CHKTEX_EXIT_ON_ERROR'} || $ENV{'CHKTEX_VALIDATE'}) {
	    # chktex doesn't let us access the error info via exit status
	    # so look through the output
	    open(my $fh, "<", "output.chktex");
	    my $errors = 0;
	    {
		local $/ = "\n";
		while(<$fh>) {
		    if (/^\S+:\d+:\d+: Error:/) {
			$errors++;
			print;
		    }
		}
	    }
	    close($fh);
	    exit(1) if $errors > 0;
	    exit(0) if $ENV{'CHKTEX_VALIDATE'};
	}
    }
}

